Interferometric Passive Radar Imaging with Deep Denoising Priors

Passive radar has key advantages over its active counterpart in terms of cost and stealth. In this paper, we address passive radar imaging problem by interferometric inversion using a spectral estimation method with a priori information within a deep learning (DL) framework. Cross-correlating the received signals from different look directions mitigates the influence of shared transmitter related phase components despite lack of a cooperative transmitter, and permits tractable inference via interferometric inversion. We thereon leverage deep architectures for modeling a priori information and for improving sample efficiency of state-of-the-art methods. Our approach comprises of an iterative algorithm based on generalizing the power method, and applies denoisers using plug-and-play (PnP) and regularization by denoising (RED) techniques. We evaluate our approach using simulated data for passive synthetic aperture radar (SAR) by using convolutional neural networks (CNN) as denoisers. The numerical experiments show that our method can achieve faster reconstruction and superior image quality in sample starved regimes than the state-of-the-art passive interferometric imaging algorithms.

==> PriorArt_DL.tex <==


\subsection{Prior Art} \textbf{\textcolor{red}{(Incomplete)}}
For imaging applications involving linear or non-linear measurement models, various prior information, such as positivity, sparsity, block sparsity etc., are commonly assumed known in advance.
For good reconstruction performance, it is important to carefully select the optimization algorithm as well as the regularization term, imposing prior information, which may not have desirable properties such as convexity, continuity, differentiability etc.
In order to avoid explicitly differentiating the regularization term, the concept of \emph{proximal operator} is implemented, which has led to a number of proximal algorithms.
Most prominent of these algorithms are the alternative direction method of multipliers (ADMM)~\cite{afonso2010fast}, and the iterative shrinkage thresholding algorithm (ISTA) and its variants~\cite{daubechies2004iterative, beck2009fast}.
\emph{Proximal operator} involves a separate optimization problem, which essentially implements a regularized denoising operation on the current estimate, where the type of regularization is defined by
%$\calR(.)$~\cite{sun2019PnP}.
prior information being imposed in the original problem.

The similarity of the \emph{proximal operator} to a denoising operation inspired the approach in~\cite{venkatakrishnan2013plug}, where the idea of replacing this operator with an image denoiser was introduced, and this technique was referred to as plug-and-play (PnP).
Various denoisers, including non-DL based ones, such as, BM3D~\cite{dabov2007image}, WNNM~\cite{gu2014weighted} etc., and DL based ones, such as, TNRD~\cite{chen2016trainable}, DnCNN~\cite{zhang2017_dncnn} can be implemented for denoising at the PnP iterations.
For an arbitrary choice of the denoiser, it may be difficult to deduce a corresponding regularization term and the associated optimization problem.
Even though the PnP concept for regularized optimization was originally introduced for the ADMM algorithm in~\cite{venkatakrishnan2013plug}, it has since combined with a range of algorithms, such as a variant of FISTA for non-linear inverse scattering~\cite{kamilov2017plug_nonlinear}, a singular value decomposition (SVD) based iterative algorithm for linear inversion under noise~\cite{awasthi2021dimensionality}, primal-dual splitting based algorithm for image restoration~\cite{ono2017primal} etc.

Additionally, a number of recent works have introduced a range of theoretical convergence results~\cite{sreehari2016PnPADMM, chan2016plug, sun2019PnP, nair2021fixed} for a number of PnP algorithms, where the forward maps are either linear or implicitly limited by the properties of the data fidelity term.
Under continuously differentiable denoisers, whose gradient is a symmetric matrix with eigenvalues between $0$ and $1$,~\cite{sreehari2016PnPADMM} establishes for the PnP-ADMM iterates that the denoiser is a proximal mapping of a proper closed convex function and the PnP algorithm converges to the global minimum.
In~\cite{sun2019PnP}, it is shown that given a convex, differentiable and Lipschitz continuous data fidelity term, $\theta$-averaged denoiser with $\theta\in(0, 1)$, and the ground truth images as fixed point to the combined gradient descent and denoising operators, PnP-ISTA converges to one of these fixed points with a rate of $\mathcal{O}(1 / t)$, where $t$ refers to the iteration number.
In~\cite{nair2021fixed}, for a special class of linear denoisers, both the convergence of the PnP iterates using ISTA and ADMM algorithms and the minimization of an explicit objective function are established.

Another line of work, related to the PnP approach, is based on the regularization by denoising (RED) framework, which was introduced in~\cite{romano2017little}.
Unlike PnP, it involves an explicit definition of the regularization term as a function of the denoiser.
In~\cite{romano2017little}, two conditions were imposed on the denoiser, namely, local homogenenity and strong passivity, both of which require the denoiser to be differentiable.
It is shown in~\cite{romano2017little} that, under these two conditions, the regularization term for RED implemented using the particular denoiser becomes convex.
%Finally, another variation of the PnP based approach is proposed in~\cite{buzzard2018_CE_SIAM}.

Similarly to the linear inversion problem, implementation of known signal priors, through convex or non-convex regularization terms, enables the recovery of structured signals from fewer number of auto-correlated measurements compared to its counterparts that ignores such prior information~\cite{soltanolkotabi2019structured}.
These improvements are expected to extend to the inversion problem using the cross-correlated measurements, as evidenced by our observation from the sparsely constrained GWF approach in~\cite{akhtar2021passive}.
Furthermore, the RED framework, proposed originally for the linear inversion problems, have been extended to the phase retrieval task in~\cite{Metzler2018_prdeep}, where the denoiser is implemented using a DnCNN network.





==> Section3A.tex <==
\subsection{Imaging Algorithms using Prior Information}
% The data model presented in~\eqref{eq:data_model}, which applies for both imaging geometries discussed in Section~\ref{sec:problem_statement} with appropriately defined $\calF$, has similarity to the one for the phaseless imaging task.
% However, unlike the current problem, the components of $\bd$ for the phaseless imaging problem results from the auto-correlated measurements instead of the cross-correlated ones.
% One of the prominent non-convex methods for phaseless imaging is the WF algorithm~\cite{candes2015phase_IEEE, yonel2020deterministic}.
% Non-convex methods are superior, in general, over their convex optimization based counterparts~\cite{candes2013phaselift, candes2015phase}, from the point of view of computational cost and memory requirement for practical applications, such as SAR imaging.
% WF algorithm and its variants~\cite{chen2015WF, zhang2017RWF, yuan2019SWF, cai2016optimalThWF, wu2020hadamardWF, kazemi2021unrolled} estimate the unknown image, given a known forward map, by implementing iterative algorithms that solve non-convex optimization problems by utilizing sophisticated initialization scheme, followed by iterative updates using the WF derivatives.
% Exact recovery guarantees have been established for the WF algorithm under Gaussian sampling vectors, coded diffraction patterns, short time Fourier transforms, and for general deterministic forward maps that satisfy a particular concentration property related to the corresponding $\calF^H\calF$ operator~\cite{yonel2020deterministic}.

Inspired by the promising results observed for the phaseless imaging problem, the generalized WF (GWF) algorithm was introduced in~\cite{yonel2019generalization} with the goal of extending the WF algorithm and its recovery guarantee to the task of recovering unknown images from cross-correlated measurements under general deterministic forward maps.
It was observed that the exact recovery of the interferometric inversion problem requires $\calF$ to satisfy a restricted isometry property (RIP), over all rank-1 positive semi-definite matrices, with a restricted isometry constant (RIC) less than $0.214$.
Similarly to the WF algorithm, GWF incorporates the spectral initialization step, modified for the cross correlated measurement model, and iterative gradient descent updates, that minimize a non-convex objective function.
More specifically, the initial image estimate, $\brho_0\in\bbC^N$, is calculated as $\sqrt{\lambda_1}\bu_1$, where $\lambda_1$ and $\bu_1$ are the leading eigenvalue-eigenvector pair of the spectral matrix, $\hat{\bX}\in\bbC^{N \times N}$.
%For the multi-static imaging configuration, $\hat{\bX}$ is calculated as follows:
%\begin{align}
%    \label{eq:GWF_spectral_matrix} \hat{\bX} & := \frac{1}{2M}\sum_{k = 1}^K\sum_{\substack{i, j = 1 \\ i \neq j}}^Sd_{i, j}(\omega_k)\ba^k_i(\ba^k_j)^H + \overline{d_{i, j}(\omega_k)}\ba^k_j(\ba^k_i)^H, \\
%    & = \calP_s(\calF^H(\bd)).
%\end{align}
$\hat{\bX}$ is defined as follows:
\begin{align}
    \label{eq:GWF_spectral_matrix} \hat{\bX} & := \calP_s(\calF^H(\bd)),
\end{align}
where $\calP_S(\bZ) := \frac{1}{2}(\bZ + \bZ^H)$ for $\bZ\in\bbC^{N \times N}$.
$\calF^H(\bd)$ is calculated
%for the multi-static imaging geometry as
%\begin{align}
%    \calF^H(\bd) & = \frac{1}{M}\sum_{k = 1}^K\sum_{\substack{i, j = 1 \\ i \neq j}}^Sd_{i, j}(\omega_k)\ba^k_i(\ba^k_j)^H.
%\end{align}
%On the other hand,
for the passive interferometric SAR imaging problem
%$\calF^H(\bd)$ is defined as
as
\begin{align}
    \calF^H(\bd) & = \frac{1}{M}\sum_{k, s = 1}^{K, S}d(\omega_k, s)\ba^{k, s}_a(\ba^{k, s}_b)^H.
\end{align}
After spectral initialization, the estimated image $\brho_l\in\bbC^N$ at the $l^{th}$ update stage is calculated using a gradient descent update, i.e.,
\begin{align}
    \brho_l & = \brho_{l - 1} - \frac{\mu_l}{\|\brho_0\|^2}\bnabla\calJ(\brho)|_{\brho = \brho_{l - 1}}.
\end{align}
$\calJ(\brho)$ refers to an objective function associated with the interferometric inversion problem.
%For the multi-static imaging problem, we refer to this objective function by $\calJ_M(\brho)$ and define it according to the following formulation:
%\begin{align}
%    \label{eq:objective_function} \calJ_M(\brho) & = \frac{1}{2M}\sum_{k = 1}^K\sum_{\substack{i, j = 1 \\ i \neq j}}^S\left[(\ba^k_i)^H\brho\brho^H\ba^k_j - d_{i, j}(\omega_k)\right]^2.
%\end{align}
%For the passive SAR imaging problem, corresponding objective function is $\calJ_P(\brho)$ can be calculated similarly as follows:
For the passive SAR received signal model in Section~\ref{sec:problem_statement}, this objective function can be calculated as follows:
%\begin{align}
%    \label{eq:objective_function_P} \calJ_P & = \frac{1}{2M}\sum_{k, s = 1}^{K, S}\left[(\ba^{k, s}_a)^H\brho\brho^H\ba^{k, s}_b - d(\omega_k, s)\right]^2.
%\end{align}
\begin{align}
    \label{eq:objective_function_P} \calJ(\brho) & = \frac{1}{2M}\sum_{k, s = 1}^{K, S}\left[(\ba^{k, s}_a)^H\brho\brho^H\ba^{k, s}_b - d(\omega_k, s)\right]^2.
\end{align}

%In~\cite{yonelTCI}, the GWF algorithm~\cite{yonel2019generalization} is applied to the multistatic radar imaging problem under Born approximation and small scene far field assumption.
%Recovery guarantee of GWF, as it relates to the isometry of the lifted forward map, is studied in the context of the relevant imaging parameters of the multistatic interferometric imaging geometry.
%It is observed that, as the central frequency and the number of receivers increase, the corresponding RIC constant of the forward map become smaller.
%Furthermore, theoretical results established that the exact recovery guarantee for multistatic interferometric imaging can be achieved under pixel spacings, that are smaller than the range resolution of the Fourier-based methods.
%Finally, the minimum sample complexity requirement was determined, which relates to number of receivers and frequency samples, for exact recovery guarantee.

%However, the GWF algorithm~\cite{yonel2019generalization} does not take into account available prior information about the unknown image class.
%In~\cite{akhtar2021passive}, a variant of the GWF algorithm is introduced for the passive multistatic radar imaging problem that incorporates sparsity prior by calculating a $k$-sparse spectral estimation, and gradient descent updates with a soft-thresholding projection operator, which is associated with $\ell_1$-norm based regularization.
%For the sparse image reconstruction problem, it is observed through numerical simulations that this sparsity constrained GWF algorithm has faster convergence rate compared to the original version that overlooks such prior information.


%\subsection{Denoising Prior based Imaging Algorithms}
However, existing implementations of the GWF algorithm for multistatic radar imaging requires a sufficiently large number of stationary receivers and high central frequency, both of which lead to increased implementation costs.
The interferometric inversion problem becomes ill-posed at low $\frac{M}{N}$ ratios as the RIP depended sufficient for exact recovery of the unconstrained GWF algorithm is not satisfied.
A way of circumventing these shortcomings while maintaining low computational cost is to apply available prior information about the unknown image class within a spectral norm maximization framework.
Such maximization problems are addressed commonly during the initial phases of the WF algorithm and its variants including the GWF algorithm to implement structured initialization steps.
We design our approach to utilize prior information about the images for attaining exact recovery via a spectral norm maximization technique from random initializations directly, and hence present an alternative to the least square minimization criteria considered by the GWF algorithm.

As specified earlier, spectral initialization involves the estimation of the leading eigenvalue-eigenvector pair of the spectral matrix $\hat{\bX}$ defined in~\eqref{eq:GWF_spectral_matrix}.
The leading eigenvector, $\bu_1\in\bbC^N$, is essentially the solution to the maximization problem $\max_{\|\bv\| = 1} \bv^H\hat{\bX}\bv$, and it is commonly estimated using the power method.
Power method is an iterative algorithm whose updates convergence to the exact $\ell_2$ normalized solution by virtue of the linear independence property of the set of its eigenvectors, and at a rate that depends on the ratio of the largest and the second largest eigenvalues.
We modify the power method to accommodate DL based prior information incorporation, and hence aim to address the following fundamental question regarding the quadratic inversion problem: under the assumption that the unknown image vectors have unit $\ell_2$ norm, can we use prior information to attain exact recovery from random initializations via a spectral norm maximization process by using a power method type algorithm?

